Document Image Coding and Clustering for Script Discrimination

The paper introduces a new method for discrimination of documents given in different scripts. The document is mapped into a uniformly coded text of numerical values. It is derived from the position of the letters in the text line, based on their typographical characteristics. Each code is considered as a gray level. Accordingly, the coded text determines a 1-D image, on which texture analysis by run-length statistics and local binary pattern is performed. It defines feature vectors representing the script content of the document. A modified clustering approach employed on document feature vector groups documents written in the same script. Experimentation performed on two custom oriented databases of historical documents in old Cyrillic, angular and round Glagolitic as well as Antiqua and Fraktur scripts demonstrates the superiority of the proposed method with respect to well-known methods in the state-of-the-art.

==> refs.tex <==
\begin{thebibliography}{10}

\bibitem{[1]} D. Ghosh, T. Dube and A. Shivaprasad, Script recognition Ð A review, IEEE Trans. Pattern Analysis and Machine Intelligence, vol.32, no.12, pp.2142-2161, 2010.

\bibitem{[2]} U. Pal and B. B. Chaudhuri, Indian script character recognition: A survey, Pattern Recognition, vol.37, no.9, pp.1887-1899, 2004.

\bibitem{[3]} N. Nagy, Twenty years of document image analysis in PAMI, IEEE Trans. Pattern Analysis and Machine Intelligence, vol.22, no.1, pp.38-62, 2000.

\bibitem{[4]} G. D. Joshi, S. Garg and J. Sivaswamy, A generalised framework for script identification, International Journal of Document Analysis and Recognition, vol.10, no.2, pp.55-68, 2007.

\bibitem{[5]} P. Sibun and A. L. Spitz, Language determination: Natural language processing from scanned document images, Proc. of the 4th Conference on Applied Natural Language Processing, Las Vegas, USA, pp.423-433, 1995.

\bibitem{[6]} A. W. Zramdini and R. Ingold, Optical font recognition using typographical features, IEEE Trans. Pattern Analysis and Machine Intelligence, vol.20, no.8, pp.877-882, 1998.

\bibitem{[7]} D. Brodi\'c, Z. N. Milivojevi\'c and \v C. A. Maluckov, An approach to the script discrimination in the Slavic documents, Soft Computing, vol.19, no.9, pp.2655-2665, 2015.

\bibitem{[8]} M. M. Galloway, Texture analysis using gray level run lengths, Computer, Graphics and Image Processing, vol.4, no.2, pp.172-179, 1975.

\bibitem{[9]} A. Chu, C. M. Sehgal and J. F. Greenleaf, Use of gray value distribution of run lengths for texture analysis, Pattern Recognition Letters, vol.11, no.6, pp.415-419, 1990.

\bibitem{[10]} B. R. Dasarathy and E. B. Holder, Image characterizations based on joint gray-level run-length distributions, Pattern Recognition Letters, vol.12, no.8, pp.497-502, 1991.

\bibitem{[11]} T. Ojala, M. Pietikainen and D. Harwood, A comparative study of texture measures with classification based on featured distributions, Pattern Recognition, vol.29, no.1, pp.51-59, 1996.

\bibitem{[12]} R. Nosaka, Y. Ohkawa and K. Fukui, Feature extraction based on co-occurrence of adjacent local binary patterns, Proc. of the 5th Pacific Rim Symposium on Image and Video Technology, Gwanju, South Korea, pp.82-91, 2011.

\bibitem{[13]} D. Brodi\'c, A. Amelio and Z. N. Milivojevi\'c, Classification of the scripts in medieval documents from Balkan region by run-length texture analysis, Proc. of the 22nd Conference on Neural Information Processing, Istanbul, Turkey, pp.442-450, 2015.

\bibitem{[14]} D. Brodi\'c, A. Amelio and Z. N. Milivojevi\'c, Characterization and distinction between closely related south Slavic languages on the example of Serbian and Croatian, Proc. of the 16th International Conference on Computer Analysis of Images and Patterns, Valletta, Malta, pp.654-666, 2015.

\bibitem{[15]} C. C. Aggarwal and C. Zhai, Mining Text Data, Springer USA, 2012.

\bibitem{[16]} N. O. Andrews and E. A. Fox, Recent Developments in Document Clustering, Tech. rep., Computer
Science, Virginia Tech., 2007.
 
\end{thebibliography}

